(LC)$^2$: LiDAR-Camera Loop Constraints For Cross-Modal Place Recognition

Localization has been a challenging task for autonomous navigation. A loop detection algorithm must overcome environmental changes for the place recognition and re-localization of robots. Therefore, deep learning has been extensively studied for the consistent transformation of measurements into localization descriptors. Street view images are easily accessible; however, images are vulnerable to appearance changes. LiDAR can robustly provide precise structural information. However, constructing a point cloud database is expensive, and point clouds exist only in limited places. Different from previous works that train networks to produce shared embedding directly between the 2D image and 3D point cloud, we transform both data into 2.5D depth images for matching. In this work, we propose a novel cross-matching method, called (LC)$^2$, for achieving LiDAR localization without a prior point cloud map. To this end, LiDAR measurements are expressed in the form of range images before matching them to reduce the modality discrepancy. Subsequently, the network is trained to extract localization descriptors from disparity and range images. Next, the best matches are employed as a loop factor in a pose graph. Using public datasets that include multiple sessions in significantly different lighting conditions, we demonstrated that LiDAR-based navigation systems could be optimized from image databases and vice versa.

==> src/figtex/fig_ablation.tex <==
%FIGURE
\begin{figure}[b]
	\centering
	\captionsetup{font=footnotesize}
	\vspace{-3mm}
	\includegraphics[width=\columnwidth]{figs/ablation}
	\caption
	{
		Effects of localizability filtering on accuracy (left upper) and the distribution of $\lambda_d$ values (left lower), in Sequence 05.
		Without threshold, our module tries place
		recognition even for images with less structural information, lowering place recognition
		performance. The sample images, their estimated depth, and localizability $\lambda_d$
		are displayed in the right column.
	}
	\label{fig:ablation}
\end{figure}
%FIGURE

==> src/figtex/fig_activation.tex <==
%FIGURE
\begin{figure}[b]
	\captionsetup{font=footnotesize}
	\vspace{-4mm}
	\centering
	\includegraphics[width=0.8\columnwidth]{figs/src/activation_cam}
	\caption
	{
		Activations of the encoder, calculated from disparity image and its localization descriptor.
		The localization descriptors were based on disparity images, but we plotted on RGB only for
		visualization. The red-colored area indicates a more sensitive area to localization descriptors,
		meaning the network focuses on that area for place recognition.
	}
	\label{fig:heatmap}
\end{figure}
%FIGURE

==> src/figtex/fig_loss.tex <==
%FIGURE
\begin{figure}[!h]
	\centering
	
	\captionsetup{font=footnotesize}
	\includegraphics[width=0.6\columnwidth]{figs/spacer/chiwawa2}
	\caption
	{
		Training Loss of our architecture. But this is dumb chiwawa.
	}
	\label{fig:loss}
	
\end{figure}
%FIGURE

